ASTA: Learning Analytical Semantics over Tables for Intelligent Data Analysis and Visualization

Intelligent analysis and visualization of tables use techniques to automatically recommend useful knowledge from data, thus freeing users from tedious multi-dimension data mining. While many studies have succeeded in automating recommendations through rules or machine learning, it is difficult to generalize expert knowledge and provide explainable recommendations. In this paper, we present the recommendation of conditional formatting for the first time, together with chart recommendation, to exemplify intelligent table analysis. We propose analytical semantics over tables to uncover common analysis pattern behind user-created analyses. Here, we design analytical semantics by separating data focus from user intent, which extract the user motivation from data and human perspective respectively. Furthermore, the ASTA framework is designed by us to apply analytical semantics to multiple automated recommendations. ASTA framework extracts data features by designing signatures based on expert knowledge, and enables data referencing at field- (chart) or cell-level (conditional formatting) with pre-trained models. Experiments show that our framework achieves recall at top 1 of 62.86% on public chart corpora, outperforming the best baseline about 14%, and achieves 72.31% on the collected corpus ConFormT, validating that ASTA framework is effective in providing accurate and explainable recommendations.

==> problem.tex <==
\label{sec:problem}


We propose a novel concept, analytical semantics over tabular data, to unearth the user motivation and common pattern behind diverse analysis and visualizations. In ~\refsec{sec:analytical_semantics}, we take conditional formatting and chart introduced in \refsec{sec:corpus} as examples to demonstrate how analytical semantics functions.
On this basis, a new research problem on data analytics and table understanding -- learning analytical semantics -- together with the recommending of conditional formatting and chart recommendation are formulated and tackled by us as machine learning tasks in \ref{sec:ml_formulation}.











==> tools.tex <==
\usepackage{xcolor}


\newcommand{\TODO}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\mengyu}[1]{\emph{\textcolor{cyan}{Mengyu: #1}}}
\newcommand{\lingbo}[1]{\emph{\textcolor{violet}{Lingbo: #1}}}
\newcommand{\tianle}[1]{\emph{\textcolor{orange}{Tianle: #1}}}
\newcommand{\xinyi}[1]{\emph{\textcolor{purple}{Xinyi: #1}}}
